On Beurling measure algebras

We show how the measure theory of regular compacted-Borel measures defined on the $\delta$-ring of compacted-Borel subsets of a weighted locally compact group $(G,\omega)$ provides a compatible framework for defining the corresponding Beurling measure algebra ${\cal M}(G,\omega)$, thus filling a gap in the literature.

==> Macros.tex <==
%mathdef2.tex - standard math definitions

\usepackage{amssymb}

% Theoremlike environments



\newtheorem{thm}{Theorem}[section]

\newtheorem{dfn}[thm]{Definition}

\newtheorem{lem}[thm]{Lemma}

\newtheorem{prop}[thm]{Proposition}

\newtheorem{remark}[thm]{Remark}

\newtheorem{cor}[thm]{Corollary}

\newtheorem{ex}[thm]{Example}

\newtheorem{question}[thm]{Question}

\newtheorem{assumption}[thm]{Assumption} 

% Macros



\def\sv{{\scriptstyle \vee}}

\def\ve{\varepsilon}
\def\sq{{\scriptscriptstyle \square}}
\def\di{\diamond}
\def\ch{\check}
\def\epg{\varepsilon_\pi G }
\def\eg{\varepsilon G}
\def\dpi{\delta_\pi}
\def\de{\delta_\varepsilon}
\def\px{\pi_\X}
\def\pe{\pi_\varepsilon}
\def\se{\sigma_\varepsilon}
\def\re{\rho_\varepsilon}

\def\stre{(\sigma \otimes \rho)_\varepsilon}

\def\pte{(\pi \otimes \pi)_\varepsilon}

\def\Pep{\Phi_{E(\pi)}}

\def\bq{\begin{question}}
\def\bt{\begin{thm}}
\def\bp{\begin{prop}}
\def\blem{\begin{lem}}
\def\bd{\begin{dfn}}
\def\br{\begin{remark}}
\def\bc{\begin{cor}}
\def\bex{\begin{ex}}
\def\beqs{\begin{eqnarray*}}
\def\beq{\begin{eqnarray}}
\def\bi{\begin{itemize}}

\def\mcb{{M_{cb}}}

\def\eq{\end{question}}
\def\et{\end{thm}}
\def\ep{\end{prop}}
\def\elem{\end{lem}}
\def\ed{\end{dfn}}
\def\er{\end{remark}}
\def\ec{\end{cor}}
\def\eex{\end{ex}}
\def\eeqs{\end{eqnarray*}}
\def\eeq{\end{eqnarray}}
\def\ei{\end{itemize}}
\def\ione{\item[(i)]}
\def\itwo{\item[(ii)]}
\def\ithree{\item[(iii)]}
\def\ifour{\item[(iv)]}
\def\ifive{\item[(v)]}
\def\isix{\item[(vi)]}

\def\wot{\widehat{\otimes}}

\def\ebwc{\preceq_{\varepsilon w}}
\def\ebc{\preceq_{\varepsilon}}
\def\wc{\preceq_{w}}
\def\qc{\preceq_{Q}}


\def\no{\noindent}
\def\ds{\displaystyle}

\def\hG{\widehat{G}}
\def\hH{\widehat{H}}
\def\ka{\kappa_\alpha}
\def\io{\iota}


\def\c{\cdot}
\def\lo{L^1(G)}
\def\lt{L^2(G)}
\def\li{L^{\infty}(G)}

\def\ov{\overline}
\def\r{\rangle}
\def\l{\langle}
\def\prep{\{ \pi, {\cal H}_\pi \} }
\def\cprep{\{ \ov{\pi}, \ov{{\H}} \} }
\def\tpi{\pi \otimes \ov{\pi}}


\def\lg{\rho_G}
\def\lh{\rho_H}

\def\GB{\mathfrak{B}}
\def\op{\overline{\phi}}

\def\H{{\cal H}}
\def\K{{\cal K}}
\def\B{{\cal{B}}} 
\def\fB{{\mathfrak B}} 
\def\CG{C^*(G)}

\def\Br{B_\rho(G)}
\def\Cr{C^*_\rho(G)}
\def\Brh{B_\rho(H)}
\def\Crh{C^*_\rho(H)}

\def\wg{W(\h{G})}
\def\wh{W(\h{H})}
\def\apg{AP(\h{G})}
\def\aph{AP(\h{H})}

\def\wug{W_u(\h{G})}
\def\wuh{W_u(\h{H})}
\def\aug{AP_u(\h{G})}
\def\auh{AP_u(\h{H})}

%\def\o{\odot}

\def\cdp{C^*_{\delta,\pi}}
\def\cpd{C^*_{\pi_d}}

\def\lhi{\rho_{H_i}}

\def\ag{{\mathfrak A}_G}
\def\ah{{\mathfrak A}_H}

\def\Hp{{\cal H}_\pi}

\def\bpa{B_{\pi \circ \alpha}}
\def\apa{A_{\pi \circ \alpha}}

\def\w*{w^*-w^*}

\def\cmg{C^*_{\rho}(M(G))}
\def\cmh{C^*_{\rho}(M(H))}

\def\msg{M^*_\rho(G)}

\def\msh{M^*_\rho(H)}

\def\brsbr{{B_\rho^*-B_\rho}}
\def\brcr{{B_\rho-C^*_\rho}}
\def\crbr{{C^*_\rho-B_\rho}}

\def\avn{{A-VN}}
\def\vna{{VN-A}}
\def\mcz{{M-C_0}}
\def\vsv{{VN^*-VN}}
\def\msm{{(M_\rho^*)^)-M_\rho^*}}

\def\CG{C^*(G)}
\def\cp{C^*_\pi}


\def\ap{A_\pi}
\def\Bp{B_\pi}



\def\xg{\X_G}
\def\xh{\X_H}
\def\xgc{\X_{G,c}}
\def\xhc{\X_{H,c}}

\def\Eg{E_G}
\def\Rg{R_G}
\def\Eh{E_H}
\def\Rh{R_H}

\def\F{{\cal F}}

\def\Af{A_\F(G)}
\def\Apif{A_{\cal PIF}(G)}


\def\thg{\theta_G}
\def\thh{\theta_H}
\def\pih{\pi_H}
\def\pig{\pi_G}

\def\ibg{\iota_{\Br}}
\def\ibh{\iota_{\Brh}}

\def\cb{\|_{cb}}

\def\ucg{UCB(\hG)}
\def\ukg{UCB_c(\hG)}
\def\ak{A_c(G)}
\def\uch{UCB(\hH)}
\def\ukh{UCB_c(\hH)}

\def\hr{\hookrightarrow}
\def\ra{\rightarrow}

\def\jin{j^{-1}}
\def\ain{\alpha^{-1}}
\def\ja{j_\alpha}
\def\jai{j_{\alpha_i}}
\def\jbi{j_{\beta_i}}

\def\vnp{VN_\pi}

\def\C{\cdot}

\def\h{\widehat}

\def\supp{{\rm supp}}

\def\hp{\h{\phi}}

\def\X{{\mathfrak X}}

\def\Y{{\mathfrak Y}}

\def\ij{{i,j}}
\def\kl{{k,l}}

\def\wt{\widetilde}
\def\od{\odot}
\def\wka{\wt{\kappa}_\alpha}

\def\oka{\ov{\kappa}_\alpha}

\def\ap{A_\pi}
\def\Ep{E_\pi}

\def\xpe{\xi*_\pi \eta}
\def\epx{\eta*_\pi \xi}

\newcommand\crep{\{ \gamma_G, \lt \} }
\newcommand\qrep{\{ \lambda_{G/H}, L^2(G/H, \mu) \} }

\newcommand\LG{\lambda_G}


\newcommand\pn{\pi_N}

\newcommand\cg{\gamma_G}
\newcommand\q{\lambda_{G/H}}

\def\aG{\alpha G}
\def\da{\delta_\alpha}
\def\pa{\omega_\alpha}
\def\ta{\theta_\alpha}

\def\vp{\varphi}
\def\DBG{\Delta(B(G))} 
\def\bs{\backslash} 

\def\bB{{\mathbb B}}
\def\bD{\Delta\!\!\!\!\Delta}

\def\O{\mathbb{O}}
\def\Q{\mathbb{Q}}


\def\gap{G^{ap}}
\def\dap{\delta^{ap}} 
\def\tdap{\widetilde{\delta^{ap}}}
\def\eap{e_{ap}}


    \def\AFG{A_\mathbbmtt{F}(G)}
    
       \def\pif{{\pi_\mathbbmtt{F}}} 

\def\PDA{{\cal P}_{\Delta(A)}} 


\def\om{\omega} 
\def\M{{\cal M}}
\def\fC{\mathfrak{C}} 
\def\fS{\mathfrak{S}} 

\def\E{{\cal E}} 
\def\L{{\cal L}}


% Disjoint Union:
\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{%
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
\newcommand{\charfusion}[3][\mathord]{
    #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}
      }
    \ifx#1\mathop\expandafter\displaylimits\fi}
\makeatother

\newcommand{\cupdot}{\charfusion[\mathbin]{\cup}{\cdot}}
\newcommand{\bigcupdot}{\charfusion[\mathop]{\bigcup}{\cdot}}

